Adding Neural Network Controllers to Behavior Trees without Destroying Performance Guarantees

In this paper, we show how Behavior Trees that have performance guarantees, in terms of safety and goal convergence, can be extended with components that were designed using machine learning, without destroying those performance guarantees. Machine learning approaches such as reinforcement learning or learning from demonstration can be very appealing to AI designers that want efficient and realistic behaviors in their agents. However, those algorithms seldom provide guarantees for solving the given task in all different situations while keeping the agent safe. Instead, such guarantees are often easier to find for manually designed model-based approaches. In this paper we exploit the modularity of behavior trees to extend a given design with an efficient, but possibly unreliable, machine learning component in a way that preserves the guarantees. The approach is illustrated with an inverted pendulum example.

==> code/name.tex <==
class Controller:

    def __init__(self, kx, kv, ktheta, komega, umax):

        # gains
        self.kx = kx
        self.kv = kv
        self.ktheta = ktheta 
        self.komega = komega

        # bounds
        self.umax = umax
        self.xmax = np.pi**2*(np.pi + self.umax)
        self.vmax = np.pi*self.umax

        # logical variables
        self.thetar = 0.0
        obj = lambda vec: vec[0]
        # eq = lambda vec: -ktheta*vec[0] - np.sin(vec[0]) - ktheta*np.arctan(kv*self.vmax + kx*self.xmax) + umax*np.cos(vec[0])
        eq = lambda vec: ktheta*vec[0] + np.sin(vec[0]) - umax*np.cos(vec[0])
        self.thetatilde = minimize(
            obj,
            [0.0],
            method='trust-constr',
            jac=grad(obj),
            hess=hessian(obj),
            bounds=[(0.0, None)],
            constraints=dict(
                type='eq',
                fun=eq,
                jac=grad(eq)
            ),
            options=dict(
                maxiter=500,
                # disp=True
            )
        )
        assert self.thetatilde.success == True
        self.thetatilde = self.thetatilde.x[0]
